An Empirical Study of Deep Learning Models for Vulnerability Detection

Deep learning (DL) models of code have recently reported great progress for vulnerability detection. In some cases, DL-based models have outperformed static analysis tools. Although many great models have been proposed, we do not yet have a good understanding of these models. This limits the further advancement of model robustness, debugging, and deployment for the vulnerability detection. In this paper, we surveyed and reproduced 9 state-of-the-art (SOTA) deep learning models on 2 widely used vulnerability detection datasets: Devign and MSR. We investigated 6 research questions in three areas, namely model capabilities, training data, and model interpretation. We experimentally demonstrated the variability between different runs of a model and the low agreement among different models' outputs. We investigated models trained for specific types of vulnerabilities compared to a model that is trained on all the vulnerabilities at once. We explored the types of programs DL may consider "hard" to handle. We investigated the relations of training data sizes and training data composition with model performance. Finally, we studied model interpretations and analyzed important features that the models used to make predictions. We believe that our findings can help better understand model results, provide guidance on preparing training data, and improve the robustness of the models. All of our datasets, code, and results are available at https://doi.org/10.6084/m9.figshare.20791240.

==> bigtable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\caption{CWE groupings}\label{fig:cwe-grouping}
\begin{tabular}{|l|l|l|}
\hline
CWE Group (example count)                          & CWE ID   & Description                                                                                        \\ \hline
\multirow{5}{*}{Buffer overflow (37291)}           & CWE-119  & Improper Restriction of Operations within the Bounds of a Memory Buffer                            \\ \cline{2-3} 
                                                   & CWE-120  & Buffer Copy without Checking Size of Input ('Classic Buffer Overflow')                             \\ \cline{2-3} 
                                                   & CWE-125  & Out-of-bounds Read                                                                                 \\ \cline{2-3} 
                                                   & CWE-129  & Improper Validation of Array Index                                                                 \\ \cline{2-3} 
                                                   & CWE-787  & Out-of-bounds Write                                                                                \\ \hline
\multirow{19}{*}{Input validation (25514)}         & CWE-134  & Use of Externally-Controlled Format String                                                         \\ \cline{2-3} 
                                                   & CWE-20   & Improper Input Validation                                                                          \\ \cline{2-3} 
                                                   & CWE-22   & Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal')                     \\ \cline{2-3} 
                                                   & CWE-354  & Improper Validation of Integrity Check Value                                                       \\ \cline{2-3} 
                                                   & CWE-426  & Untrusted Search Path                                                                              \\ \cline{2-3} 
                                                   & CWE-494  & Download of Code Without Integrity Check                                                           \\ \cline{2-3} 
                                                   & CWE-502  & Deserialization of Untrusted Data                                                                  \\ \cline{2-3} 
                                                   & CWE-59   & Improper Link Resolution Before File Access ('Link Following')                                     \\ \cline{2-3} 
                                                   & CWE-601  & URL Redirection to Untrusted Site ('Open Redirect')                                                \\ \cline{2-3} 
                                                   & CWE-611  & Improper Restriction of XML External Entity Reference                                              \\ \cline{2-3} 
                                                   & CWE-706  & Use of Incorrectly-Resolved Name or Reference                                                      \\ \cline{2-3} 
                                                   & CWE-74   & Improper Neutralization of Special Elements in Output Used by a Downstream Component ('Injection') \\ \cline{2-3} 
                                                   & CWE-77   & Improper Neutralization of Special Elements used in a Command ('Command Injection')                \\ \cline{2-3} 
                                                   & CWE-78   & Improper Neutralization of Special Elements used in an OS Command ('OS Command Injection')         \\ \cline{2-3} 
                                                   & CWE-79   & Improper Neutralization of Input During Web Page Generation ('Cross-site Scripting')               \\ \cline{2-3} 
                                                   & CWE-89   & Improper Neutralization of Special Elements used in an SQL Command ('SQL Injection')               \\ \cline{2-3} 
                                                   & CWE-90   & Improper Neutralization of Special Elements used in an LDAP Query ('LDAP Injection')               \\ \cline{2-3} 
                                                   & CWE-93   & Improper Neutralization of CRLF Sequences ('CRLF Injection')                                       \\ \cline{2-3} 
                                                   & CWE-94   & Improper Control of Generation of Code ('Code Injection')                                          \\ \hline
\multirow{31}{*}{Privilege escalation (32749)}     & CWE-1021 & Improper Restriction of Rendered UI Layers or Frames                                               \\ \cline{2-3} 
                                                   & CWE-200  & Exposure of Sensitive Information to an Unauthorized Actor                                         \\ \cline{2-3} 
                                                   & CWE-209  & Generation of Error Message Containing Sensitive Information                                       \\ \cline{2-3} 
                                                   & CWE-254  & CWE CATEGORY: 7PK - Security Features                                                              \\ \cline{2-3} 
                                                   & CWE-255  & CWE CATEGORY: Credentials Management Errors                                                        \\ \cline{2-3} 
                                                   & CWE-264  & CWE CATEGORY: Permissions, Privileges, and Access Controls                                         \\ \cline{2-3} 
                                                   & CWE-269  & Improper Privilege Management                                                                      \\ \cline{2-3} 
                                                   & CWE-281  & Improper Preservation of Permissions                                                               \\ \cline{2-3} 
                                                   & CWE-284  & Improper Access Control                                                                            \\ \cline{2-3} 
                                                   & CWE-285  & Improper Authorization                                                                             \\ \cline{2-3} 
                                                   & CWE-287  & Improper Authentication                                                                            \\ \cline{2-3} 
                                                   & CWE-290  & Authentication Bypass by Spoofing                                                                  \\ \cline{2-3} 
                                                   & CWE-295  & Improper Certificate Validation                                                                    \\ \cline{2-3} 
                                                   & CWE-310  & CWE CATEGORY: Cryptographic Issues                                                                 \\ \cline{2-3} 
                                                   & CWE-311  & Missing Encryption of Sensitive Data                                                               \\ \cline{2-3} 
                                                   & CWE-320  & CWE CATEGORY: Key Management Errors                                                                \\ \cline{2-3} 
                                                   & CWE-327  & Use of a Broken or Risky Cryptographic Algorithm                                                   \\ \cline{2-3} 
                                                   & CWE-330  & Use of Insufficiently Random Values                                                                \\ \cline{2-3} 
                                                   & CWE-331  & Insufficient Entropy                                                                               \\ \cline{2-3} 
                                                   & CWE-345  & Insufficient Verification of Data Authenticity                                                     \\ \cline{2-3} 
                                                   & CWE-346  & Origin Validation Error                                                                            \\ \cline{2-3} 
                                                   & CWE-347  & Improper Verification of Cryptographic Signature                                                   \\ \cline{2-3} 
                                                   & CWE-352  & Cross-Site Request Forgery (CSRF)                                                                  \\ \cline{2-3} 
                                                   & CWE-358  & Improperly Implemented Security Check for Standard                                                 \\ \cline{2-3} 
                                                   & CWE-522  & Insufficiently Protected Credentials                                                               \\ \cline{2-3} 
                                                   & CWE-532  & Insertion of Sensitive Information into Log File                                                   \\ \cline{2-3} 
                                                   & CWE-668  & Exposure of Resource to Wrong Sphere                                                               \\ \cline{2-3} 
                                                   & CWE-693  & Protection Mechanism Failure                                                                       \\ \cline{2-3} 
                                                   & CWE-732  & Incorrect Permission Assignment for Critical Resource                                              \\ \cline{2-3} 
                                                   & CWE-862  & Missing Authorization                                                                              \\ \cline{2-3} 
                                                   & CWE-918  & Server-Side Request Forgery (SSRF)                                                                 \\ \hline
\multirow{14}{*}{Resource allocation/free (33748)} & CWE-399  & CWE CATEGORY: Resource Management Errors                                                           \\ \cline{2-3} 
                                                   & CWE-400  & Uncontrolled Resource Consumption                                                                  \\ \cline{2-3} 
                                                   & CWE-404  & Improper Resource Shutdown or Release                                                              \\ \cline{2-3} 
                                                   & CWE-415  & Double Free                                                                                        \\ \cline{2-3} 
                                                   & CWE-416  & Use After Free                                                                                     \\ \cline{2-3} 
                                                   & CWE-476  & NULL Pointer Dereference                                                                           \\ \cline{2-3} 
                                                   & CWE-664  & Improper Control of a Resource Through its Lifetime                                                \\ \cline{2-3} 
                                                   & CWE-665  & Improper Initialization                                                                            \\ \cline{2-3} 
                                                   & CWE-763  & Release of Invalid Pointer or Reference                                                            \\ \cline{2-3} 
                                                   & CWE-769  & DEPRECATED: Uncontrolled File Descriptor Consumption                                               \\ \cline{2-3} 
                                                   & CWE-770  & Allocation of Resources Without Limits or Throttling                                               \\ \cline{2-3} 
                                                   & CWE-772  & Missing Release of Resource after Effective Lifetime                                               \\ \cline{2-3} 
                                                   & CWE-824  & Access of Uninitialized Pointer                                                                    \\ \cline{2-3} 
                                                   & CWE-909  & Missing Initialization of Resource                                                                 \\ \hline
\multirow{12}{*}{Value propagation errors (15126)} & CWE-172  & Encoding Error                                                                                     \\ \cline{2-3} 
                                                   & CWE-189  & CWE CATEGORY: Numeric Errors                                                                       \\ \cline{2-3} 
                                                   & CWE-19   & CWE CATEGORY: Data Processing Errors                                                               \\ \cline{2-3} 
                                                   & CWE-190  & Integer Overflow or Wraparound                                                                     \\ \cline{2-3} 
                                                   & CWE-191  & Integer Underflow (Wrap or Wraparound)                                                             \\ \cline{2-3} 
                                                   & CWE-252  & Unchecked Return Value                                                                             \\ \cline{2-3} 
                                                   & CWE-369  & Divide By Zero                                                                                     \\ \cline{2-3} 
                                                   & CWE-617  & Reachable Assertion                                                                                \\ \cline{2-3} 
                                                   & CWE-674  & Uncontrolled Recursion                                                                             \\ \cline{2-3} 
                                                   & CWE-682  & Incorrect Calculation                                                                              \\ \cline{2-3} 
                                                   & CWE-704  & Incorrect Type Conversion or Cast                                                                  \\ \cline{2-3} 
                                                   & CWE-835  & Loop with Unreachable Exit Condition ('Infinite Loop')                                             \\ \hline
\end{tabular}
\end{table}







==> code-features.tex <==



\begin{enumerate}
\item group: \verb|macros|
\begin{itemize}
	\item \verb|preproc_ifdef|
	\item \verb|preproc_if|
	\item \verb|preproc_function_def|
	\item \verb|preproc_arg|
	\item \verb|preproc_params|
	\item \verb|preproc_def|
	\item \verb|preproc_else|
	\item \verb|preproc_defined|
	\item \verb|preproc_call|
	\item \verb|preproc_directive|
	\item \verb|preproc_elif|
\end{itemize}
\item \verb|__asm__|
\item \verb|lexical.num_chars|
\item group: \verb|pointer dereference|
\begin{itemize}
	\item \verb|field_expression|
	\item \verb|pointer_expression|
\end{itemize}
\item group: \verb|array dereference|
\begin{itemize}
	\item \verb|subscript_designator|
	\item \verb|subscript_expression|
\end{itemize}
\item \verb|for_statement|
\item group: \verb|while/do-while|
\begin{itemize}
    \item \verb|while_statement|
    \item \verb|do_statement|
\end{itemize}
\item \verb|call_expression|
\item \verb|if_statement|
\item group: \verb|control-flow jumps|
\begin{itemize}
    \item \verb|break_statement|
    \item \verb|continue_statement|
    \item \verb|return_statement|
\end{itemize}
\item group: \verb|unstructured control-flow|
\begin{itemize}
    \item \verb|labeled_statement|
    \item \verb|goto_statement|
\end{itemize}
\item group: \verb|switch/case|
\begin{itemize}
    \item \verb|switch_statement|
    \item \verb|case_statement|
\end{itemize}
\item \verb|comment|
\end{enumerate}

==> discussion.tex <==
\begin{listing}
    \begin{minted}[escapeinside=@@,breaklines,fontsize=\footnotesize,breakanywhere,linenos,highlightcolor=yellow!50,highlightlines={1,2,5,10,11,15,17},numbersep=3pt]{C}
static int of_dpa_cmd_add_l2_flood(OfDpa *of_dpa, OfDpaGroup *group, //*
    RockerTlv **group_tlvs) //*
{
//...4 lines
     if (!group_tlvs[ROCKER_TLV_OF_DPA_GROUP_COUNT] || //*
         !group_tlvs[ROCKER_TLV_OF_DPA_GROUP_IDS]) {
         return -ROCKER_EINVAL;
     }
     group->l2_flood.group_count =
         rocker_tlv_get_le16(group_tlvs[ROCKER_TLV_OF_DPA_GROUP_COUNT]); //*
@\diffremove{-    tlvs = g\_malloc0((group-{\textgreater}l2\_flood.group\_count + 1)}@ //*
@\diffremove{-                     sizeof(RockerTlv *));}@
@\diffadd{+    tlvs = g\_new0(RockerTlv *, group-{\textgreater}l2\_flood.group\_count + 1);}@
//...3 lines
     g_free(group->l2_flood.group_ids);
     group->l2_flood.group_ids = //*
@\diffremove{-    g\_malloc0(group-{\textgreater}l2\_flood.group\_count * sizeof(uint32\_t));}@ //*
@\diffadd{+    g\_new0(uint32\_t, group-{\textgreater}l2\_flood.group\_count);}@
//...36 lines
    \end{minted}
    \caption{Devign example 2846 (qemu): vulnerable code which was correctly predicted by \wip{6} models. \colorbox{yellow!50}{\mystrut(5,0){\ }} = top-10 lines in common by the majority of models. \wip{TODO: Skip line numbers so that they are accurate to the complete code listing}}
    \label{lst:buggy-correct-gnew}
\end{listing}

\section{Discussions}\label{sec:actionables}
what else we have tried but are not very successful.

We have done a broader investigation beyond the RQs documented. We reported the experience. We hope this section is equivelent ly to be useful.


\begin{itemize}
    \item not the dataset size, but the quality of the data, other arhicteucre
\end{itemize}


Given an architecuture, but different architecture can fail.

\begin{itemize}
\item data improvement (hard data, cleaning data)
\item representation analysis
\end{itemize}



Failed effort: 

representation analysis

manual inspections 

Our goal is not to reproduce but investigating 


{\bf RQ.B3} What are the noisy data? How can we find them? %what are the performance improvement after we remove the bad data?

\vspace{0.2cm}
\noindent{\bf Motivation:} It is known that the datasets used for deep learning based vulnerability detection can be noisy ~\cite{are_we_there_yet}. Recent research has demonstrated that by using semantic information, removing duplicated data, and balancing the dataset distributions can improve performance by 33.57\% and 128.38\%~\cite{are_we_there_yet}. However, given a very large dataset, it is very challenging to validate individual data points, especially \ben{because many of such projects cannot build;} the traditional techniques of program analysis and testing do not apply here.  During our study, we found a case where two functions with different names, and the function bodies are equivalent, containing only a {\tt return;} statement. However, the model predicts the two examples with one {\it vulnerable} and the other {\it non-vulnerable}. This inspired our approach: define a set of templates of non-vulnerable data and check their labels and the output of the models.

\noindent{\bf Study Setup:}
{\color{blue} 
During analyses of different models and their representation ouputs, certain groups of function examples stoodout as problematic. We characterized these into groups seen in table \ref{tab1}
Both the MSR and devign datasets were analyzed using tree-sitter\footnote{https://tree-sitter.github.io/tree-sitter/} to build an AST representation of each datapoint. Based on the AST structure, functions were identified as not having enough information to determine whether the function itself is vulnerable or not. Currently our analyses is strict for finding such examples to avoid the risk of flagging good examples, thus more examples do exist. LIST EXAMPLES?}

\noindent{\bf Findings:}

\begin{table}[htbp]
\caption{Non-Vulnerable Data and Their Incorrect Labels}
\begin{center}
\begin{tabular}{|l||l|c|c|}
\hline
Type   & Count  & Incorrect label & Incorrect pred\\\hline\hline
Return only      & 2552  &  74 & 67.11 \\\hline
Empty func       & 1804 & 62 & 31.33\\\hline
Comment only     & 59 & 3 & 2.67 \\\hline
Identifier only & 13 & 2 & 1.22\\\hline
Print only       & 2 & 0 & 0\\\hline 
%Total functions & 215954 & \% \\\hline
%Total           & 2.05\% & 0.07\% \\\hline





\end{tabular}
\label{tab1}
\end{center}
\end{table}



{\color{blue} Table \ref{tab1} shows the type of function and the count for both MSR and devign. Of those examples there were incorrect labels on 0.07\% of all examples. CodeBERT, PLBART and ReGVD showed that on these reported datapoints the average across 3 seeds for 3 models (9 total runs) the average incorrect predictions among the set of problematic datapoints.
Models for CodeBERT, PLBART and LineVul were then retrained using the filtered MSR and devign datasets to determine the performance impact of including/excluding such examples. Given the small number of examples the 3 models did not see any significant changes in performance. 

 We show bad data exists. This is a first step to help validate the data. We show 
 
 What is the consequence of the noisy data?}

==> listings.tex <==
% \newcommand{\highlight}[1]{\colorbox{yellow!50}{#1}}
\newcommand{\highlight}[1]{#1} % use minted highlighting because it wraps correctly
\newcommand{\diffadd}[1]{\textcolor{green!60!black}{#1}}
\newcommand{\diffremove}[1]{\textcolor{red}{#1}}
\def\mystrut(#1,#2){\vrule height #1pt depth #2pt width 0pt} % https://tex.stackexchange.com/a/14604

%%%%%%%
% SUCCESS MEMORY LEAK 6543
%%%%%%%
\begin{listing}
    % \begin{minted}[escapeinside=@@,breaklines,fontsize=\small,linenos,highlightcolor=yellow!50,highlightlines={2,6,7,10,14,17,18,19,20,22}]{C}
    \begin{minted}[escapeinside=@@,breaklines,fontsize=\footnotesize,breakanywhere,linenos,highlightcolor=yellow!50,highlightlines={1,5,6,9,13,16,17,18,19,21},numbersep=3pt]{C}
static int asf_read_ext_content(AVFormatContext *s, const GUIDParseTable *g) // (3)
{
    ASFContext *asf  = s->priv_data;
    AVIOContext *pb  = s->pb;
    @\highlight{uint64\_t size    = avio\_rl64(pb);}@ //(7)
    @\highlight{uint16\_t nb\_desc = avio\_rl16(pb);}@ //(8)
    int i, ret;
    for (i = 0; i < nb_desc; i++) {
        @\highlight{uint16\_t name\_len, type, val\_len;}@ //(5)
        uint8_t *name = NULL;
        name_len = avio_rl16(pb);
        if (!name_len)
            @\highlight{return AVERROR\_INVALIDDATA;}@ //(6)
        name = av_malloc(name_len);
        if (!name)
            @\highlight{return AVERROR(ENOMEM);}@ //(9)
        @\highlight{avio\_get\_str16le(pb, name\_len, name,}@ //(4)
                         @\highlight{name\_len);}@ //(2)
        @\highlight{type    = avio\_rl16(pb);}@ //(10)
        val_len = avio_rl16(pb);
        @\diffremove{\highlight{if ((ret = process\_metadata(s, name, name\_len, val\_len, type, \&s->metadata)) < 0)}}@ //(1)
        @\diffadd{ret = process\_metadata(s, name, name\_len, val\_len, type, \&s->metadata);}@
        @\diffadd{av\_freep(&name);}@
        @\diffadd{if (ret < 0)}@
            return ret;
    }
    align_position(pb, asf->offset, size);
    return 0;
}

    \end{minted}
    \caption{Memory leak successfully detected by LineVul. The top-10 lines reported by LIT are highlighted in yellow.}
    \label{lst:linevul-memoryleak-success}
\end{listing}

%%%%%%%
% FAILURE MEMORY LEAK 262
%%%%%%%
% \begin{listing}
%     \begin{minted}[escapeinside=@@,breaklines,fontsize=\small,linenos,highlightcolor=yellow!50,highlightlines={2,7,10,12,18,19,20,22,24,25,28}]{C}
% // commit message FFmpeg 964f07f68e (target=1, prob=0.9990613, correct=True): hevc: Fix memory leak related to a53_caption data
% @\highlight{static av\_cold int hevc\_init\_context(AVCodecContext *avctx)}@ //(6)
% {
%     HEVCContext *s = avctx->priv_data;
%     int i;
%     s->avctx = avctx;
%     @\highlight{s->HEVClc = av\_mallocz(sizeof(HEVCLocalContext));}@ //(2)
%     if (!s->HEVClc)
%         goto fail;
%     @\highlight{s->HEVClcList[0] = s->HEVClc;}@ //(5)
%     s->sList[0] = s;
%     @\highlight{s->cabac\_state = av\_malloc(HEVC\_CONTEXTS);}@ //(3)
%     if (!s->cabac_state)
%         goto fail;
%     s->output_frame = av_frame_alloc();
%     if (!s->output_frame)
%         goto fail;
%     @\highlight{for (i = 0; i < FF\_ARRAY\_ELEMS(s->DPB); i++) \{}@ //(0)
%         @\highlight{s->DPB[i].frame = av\_frame\_alloc();}@ //(4)
%         @\highlight{if (!s->DPB[i].frame)}@ //(8)
%             goto fail;
%         @\highlight{s->DPB[i].tf.f = s->DPB[i].frame;}@ //(1)
%     }
%     s->max_ra = INT_MAX;
%     @\highlight{s->md5\_ctx = av\_md5\_alloc();}@ //(9)
%     if (!s->md5_ctx)
%         goto fail;
%     @\highlight{ff\_bswapdsp\_init(&s->bdsp);}@ //(7)
%     s->context_initialized = 1;
%     s->eos = 0;

%   @\diffadd{ff\_hevc\_reset\_sei(s);}@
    
%     return 0;
% fail:
%     hevc_decode_free(avctx);
%     return AVERROR(ENOMEM);
% }
%     \end{minted}
%     \caption{An example of a failed memory leak detection by LineVul. Allocations of fields on \texttt{s} are highlighted as if detecting a memory leak, but the leaky field is \texttt{a53\_caption} (freed in \texttt{ff\_hevc\_reset\_set(s)}). Green = added in vulnerability-fixing commit, red = removed in VFC, yellow = top-10 most important according to interpretability model.}
%     \label{lst:linevul-memoryleak-success}
% \end{listing}



%%%%%%%
% FAILURE GNEW 2846
%%%%%%%
% ,breaksymbolleft=


%%%%%%%
% FAILURE SPURIOUS 1628
%%%%%%%




%%%%%%%
% EXAMPLE
%%%%%%%
% \begin{listing}
%     \begin{minted}[escapeinside=@@,breaklines,fontsize=\small,linenos,highlightcolor=yellow!50,highlightlines={}]{C}
%     \end{minted}
%     \caption{A code listing}
%     \label{}


==> logistic_regression.tex <==

We trained a Logistic Regression (LR) model on the above dataset to predict which code features were hard or easy for the NN model.

$$p(x) = \sigma(\beta_0 + \beta_1 x_1 + \ldots + 
\beta_n x_n)$$

$\beta_0, \beta_1, \ldots, \beta_F$ are a set of coefficients. $\beta_0$ is an intercept.  $p(x)$ denotes the probability that the model predicts x correctly.  $\Sigma_i^n x_i * \beta_i$ indicates the contribution of the term, thus the importance, to the prediction. 

We built a model to classify the failure dataset (label 0) from the successful dataset (label 1) for a trained deep learning model.  The important features a deep learning uses that distinguish failure and successful datasets are the components that made important contributions $Importance_x = \Sigma_j^n x_n * \beta_n$.



Learn what features are present in the failure dataset, what features are present in the successful dataset.

Here we use machine learning to explore whether we can use the code features to build a model to predict if a NN model can predict correctly.  p(x)<0.5, the model will predict incorrectly, p(x)>0.5 the model will predict correctly.

which represents the prior probability that $correct(x) = 1$. Each coefficient $\beta_1, \ldots, \beta_F$ corresponds to the predicted odds ratio of one code feature.
The model outputs a probability $p(x)$ denoting the probability that $correct(x) = 1$, which is calculated by the following formula:
, where $\sigma$ is the sigmoid function.
Based on the LR model coefficients, we output a binary value $\hat{correct}(x) = \begin{cases}
  1  & p(x) \geq 0.5 \\
  0 & p(x) < 0.5
\end{cases}$.
For each example $x$, i.e. a function, in the dataset, $x_i$ denotes the count of the $i^{th}$ code feature in the example.

We quantified the difficulty of an example $x$ according to the following function: $Difficulty_x = \Sigma_j^F x_j * \beta_j$.

Steps of the experiment:

\begin{enumerate}
    \item Train LR model on validation set to predict NN model correctness based on a list of code features.
    
    \item \wei{Use feature reduction techniques such as MRMR, forward, backward feature selections to build a most accurate model}
    % Feature selection methods: 
    % \begin{enumerate}
    %     \item Run univariate analysis for each code feature, noting the significance (P-value) output by the statistical model. Choose the code features which meet a significance threshold P $>$ 0.10.
    %     \item Use stepwise forward regression or stepwise backward regression to select the most important features.
    %     \item Consider scientific plausibility of the features and remove features which are not plausibly connected to the dependent variable.
    %     \item For features which are highly correlated, such as len and num\_expressions, remove the least significant one. This is because using two highly correlated features dilutes the association to each one.
    %     \item Remove features from consideration that appear in e.g. $<$1\% of the data. For these, the LR model will not be able to learn a meaningful association.
    %     % \item Consider that the direction of the association may not be uniform. For this reason the LR model may not pick up some associations.
    % \end{enumerate}
    \item Validate LR model.
    \begin{itemize}
        \item Validate that the LR model's accuracy on test set is adequate (above a subjective threshold and above random baseline).
        \item Validate that the LR model's confidence interval on parameters is not too large.
        \item Choose hard/easy examples from the test set and evaluate NN model. We expect NN model to perform better on easy set and worse on hard set.
    \end{itemize}
    \item Use coefficients from LR model to explain which code features are hardest/easiest for the model.

    
    \item Analyze NN model performance on hard/easy datasets across different NN models, discuss results.
    \item Hypothesis: Programs with certain code features are hard to learn for all models. Some models consider some code features especially hard to learn.
\end{enumerate}
